Active Self-Assembly of Algorithmic Shapes and Patterns in Polylogarithmic Time

We describe a computational model for studying the complexity of self-assembled structures with active molecular components. Our model captures notions of growth and movement ubiquitous in biological systems. The model is inspired by biology's fantastic ability to assemble biomolecules that form systems with complicated structure and dynamics, from molecular motors that walk on rigid tracks and proteins that dynamically alter the structure of the cell during mitosis, to embryonic development where large-scale complicated organisms efficiently grow from a single cell. Using this active self-assembly model, we show how to efficiently self-assemble shapes and patterns from simple monomers. For example, we show how to grow a line of monomers in time and number of monomer states that is merely logarithmic in the length of the line. Our main results show how to grow arbitrary connected two-dimensional geometric shapes and patterns in expected time that is polylogarithmic in the size of the shape, plus roughly the time required to run a Turing machine deciding whether or not a given pixel is in the shape. We do this while keeping the number of monomer types logarithmic in shape size, plus those monomers required by the Kolmogorov complexity of the shape or pattern. This work thus highlights the efficiency advantages of active self-assembly over passive self-assembly and motivates experimental effort to construct general-purpose active molecular self-assembly systems.

==> mainresults.tex <==
%


%
\section{Main results}

We are interested in the time complexity and program size complexity (measured by the number of distinct monomer states) for an assembly  system that uniquely produces a prescribed shape from a single seed monomer. We begin by showing that a line can be quickly grown using few states. 
\begin{theorem}[Synchronized line]\label{thm:sync}
In time $O(\log n)$, with $O(\log n)$ states, a line of length $n \in \mathbb{N}$ can be uniquely produced in such a way that each {\nut}  switches to a prescribed final state, but only after all insertions on the line have finished. 
\end{theorem}
The proof is in Section~\ref{sect:chain}. The efficient line construction  forms the basis of our two main results on shape and pattern computation.  %

Firstly, we show that arbitrary connected two-dimensional geometric shapes with~$n$ pixels can be constructed in expected time $O(\log^2 n +  t(n) \log n)$ using $O(\log n + s)$ states, where $t(n)$ is the time required for a program-size $s$ Turing machine to determine if a given pixel is in the shape. 


%

\begin{theorem}\label{thm:shape}
An arbitrary connected computable 2D shape of size $\leq \sqrt{n} \times \sqrt{n}$ can be  constructed in expected time $O(\log^2 n + t(|n|)) $  using  $O(s + \log n)$ states. Here, $t(|n|)$ is the time required for a program-size $s$ Turing machine to compute, given the index of a pixel $n$, whether the pixel is present in the shape. 
\end{theorem}
Here, $|n| = \lceil \log_2 n \rceil$ is the length of binary string encoding $n \in \mathbb{N}$. The proof is contained  in Section~\ref{sect:complexityOne}.

For complicated shapes, the main bottleneck here is Turing machine time, so we look to $n \times n$ patterns, whose pixels are computable by Turing machines that run in time  polynomial in their input size (which is polylogarithmic in $n$ here). It turns out that such patterns are computable in the model in time polylogarithmic in $n$ using only $O(\log n + s)$ states. Also, these patterns can be computed without growing outside the pattern's $n \times n$  boundary. Furthermore, this works  in  a distributed asynchronous fashion, using very few monomer states, and using only short-range local communication over distances logarithmic in shape size.


%

\begin{theorem}
An arbitrary finite computable 2D pattern of size $\leq n \times n$, where $n = 2^{2^p}, p\in \mathbb{N}$, with pixels whose color is computable on a  polynomial  time $O(\log^{\ell} n)$, linear space  $O(|n|)$, program-size $s$ Turing machine, can be constructed  in expected time %
$O(\log^{\ell+1} n)$, with $O(s + \log n)$ monomer states and without growing outside the pattern borders. Moreover,  this can be done  without explicitly using synchronization.
\end{theorem}
The proof is contained in Section \ref{sect:pattern}.




